Under the Underground: Predicting Private Interactions in Underground Forums

Underground forums where users discuss, buy, and sell illicit services and goods facilitate a better understanding of the economy and organization of cybercriminals. Prior work has shown that in particular private interactions provide a wealth of information about the cybercriminal ecosystem. Yet, those messages are seldom available to analysts, except when there is a leak. To address this problem we propose a supervised machine learning based method able to predict which public \threads will generate private messages, after a partial leak of such messages has occurred. To the best of our knowledge, we are the first to develop a solution to overcome the barrier posed by limited to no information on private activity for underground forum analysis. Additionally, we propose an automate method for labeling posts, significantly reducing the cost of our approach in the presence of real unlabeled data. This method can be tuned to focus on the likelihood of users receiving private messages, or \threads triggering private interactions. We evaluate the performance of our methods using data from three real forum leaks. Our results show that public information can indeed be used to predict private activity, although prediction models do not transfer well between forums. We also find that neither the length of the leak period nor the time between the leak and the prediction have significant impact on our technique's performance, and that NLP features dominate the prediction power.

==> sec/sk-oldreses.tex <==

\subsection{Carders Information}

We have public messages for all these forums. But the private messages are where commerce takes place. So can we figure out what prompts a private message? Can we figure out what the private map will look like. 

\begin{enumerate}

\item{} How different are the public and private graphs?
	\begin{enumerate}

	\item{} There are lots of ways to build the public graph. The private graph is pretty straightforward. Nodes are users, edges represent if a message was sent/how many messages were sent. The public graph is more complicated. How do we make connections. 	
		\begin{enumerate}
		\item{}  Connect everyone who talks in the same thread.
		\item{}  Connect the thread owner with everyone in the thread
		\item{} Connect everyone who directly replies to a post/comment
		\end{enumerate}
	\item{} Comparing the graphs.
	\begin{enumerate}
		\item{}Total public connections (edges): 603,600. Total public threads: 373,143.

		\item{}Total private connections (edges): 40,797. Total private messages: 197,067

		\item{}96.3\% (581,372/603,600) of users who participated in the same public thread never send private messages. The remaining 3.7\% sent private messages.

		\item{}45.5\% (18,569/40,797) of private connections never participated in the same public thread. The remaining 54.5\% did comment in the same thread at some point. 

		\item{}The average number of private messages sent between users \emph{without} public connections is 3.579 (66,463 messages and 18,569 private connections)

		\item{}The average number of private messages sent between users \emph{with} public connections is 5.817 (129,292 messages and 22,228 private connections)

	\end{enumerate}

	
	\end{enumerate}
\item{} What public connections trigger private ones?

	\begin{enumerate}
	\item{}I compiled a list that spawn public posts and a list of those that don't. 
	\item{}What features should we use in an ML problem? Is there literature on similar problems? Is bag of words enough?
	\item{}What classifier should we use?
	\item{}Do [b][s] posts imply a private messages better? 
		\begin{enumerate}
		\item{}11.00\% (66,416/603,600) of public connections are in a thread tagged as [B], [S], or both. 16.38\% (61,125/373,143) of \emph{threads} are tagged as [B], [S], or both.

		\item{}89.48\% (59,433/66,416) of public conversations (pairs) never participated in the same thread containing the flag [B] or [S] or both. The remaining 10.51\% participated in the same thread containing the flag [B] or [S] or both.

		\end{enumerate}
	\end{enumerate}
	


\end{enumerate}

 



%\maketitle
\subsection{Upper Bound Metrics: Carders}
This sections contains information about the differences between the public and private messages. The goal is to predict an upper bound for how well we can form the private graph given the public. To do this, we take all of the private connections and determine if there is a possible connection in the public graph.

\begin{description}
\item[ -] Total public connections (edges): 603,600. Total public threads: 373,143.

\item[ -] Total private connections (edges): 40,797. Total private messages: 197,067

\item[ -] 96.3\% (581,372/603,600) of users who participated in the same public thread never send private messages. The remaining 3.7\% sent private messages.

\item[ -] 45.5\% (18,569/40,797) of private connections never participated in the same public thread. The remaining 54.5\% did comment in the same thread at some point. 

\item[ -] 11.00\% (66,416/603,600) of public connections are in a thread tagged as [B], [S], or both. 16.38\% (61,125/373,143) of \emph{threads} are tagged as [B], [S], or both.

\item[ -] 89.48\% (59,433/66,416) of public conversations (pairs) never participated in the same thread containing the flag [B] or [S] or both. The remaining 10.51\% participated in the same thread containing the flag [B] or [S] or both.

\item[ -] The average number of private messages sent between users \emph{without} public connections is 3.579 (66,463 messages and 18,569 private connections)

\item[ -] The average number of private messages sent between users \emph{with} public connections is 5.817 (129,292 messages and 22,228 private connections)

\end{description}

